3D Finite Element Modeling of Current Densities in Semiconductor Transport with Impact Ionization

In this article we propose two novel 3D finite element models, denoted method A and B, for electron and hole Drift-Diffusion (DD) current densities. Method A is based on a primal-mixed formulation of the DD model as a function of the quasi-Fermi potential gradient, while method B is a modification of the standard DD formula based on the introduction of an artificial diffusion matrix. Both methods are genuine 3D extensions of the classic 1D Scharfetter-Gummel difference formula. The proposed methods are compared in the 3D simulation of a p-n junction diode and of a p-MOS transistor in the on-state regime. Results show that method A provides the best performance in terms of physical accuracy and numerical stability. Method A is then used in the 3D simulation of a n-MOS transistor in the off-state regime including the impact ionization generation mechanism. Results demonstrate that the model is able to accurately compute the I-V characteristic of the device until drain-to-bulk junction breakdown.

==> commands.tex <==
%% OPTIONAL MACRO DEFINITIONS
\newcommand{\paren}[1]{\left(#1\right)}
\newcommand{\D}[2]{\dfrac{d#1}{d#2}}
\newcommand{\PD}[2]{\dfrac{\partial#1}{\partial#2}}
\newcommand{\PDD}[3]{\dfrac{\partial^{#1}{#2}}{\partial{#3}^{#1}}}
\newcommand{\lap}[1]{\Delta #1}
\newcommand{\at}[2]{\left. #1 \right|_{#2}}
\newcommand{\grad}[1]{\boldsymbol{\nabla} #1}
\newcommand{\mb}[1]{\mathbf{#1}}
\newcommand{\bm}[1]{\boldsymbol{#1}}
\newcommand{\abs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\norm}[1]{\left\lVert #1 \right\rVert}
\newcommand{\dual}[2]{\left\langle #1,#2 \right\rangle}
%\newcommand{\Int}[2]{\displaystyle{\int\limits_{#1}^{#2}}}
\newcommand{\Int}[1]{\displaystyle{\int\limits_{#1}}}
%\newcommand{\R}{\mathbb{R}}

\newcommand{\jumpl} {\left[\!\left[}
\newcommand{\jumpr} {\right]\!\right]}
\newcommand{\jmp}[1]{\,[\![#1]\!]}

\newcommand{\Div}{\text{div}\,}
\newcommand{\nabu}{\boldsymbol{\nabla}\,}
\newcommand{\vect}[1]{\bm{#1}}

\newcommand{\Th}{\mathcal{T}_h}
\newcommand{\Eh}{\mathcal{E}_h}

\def\x{\mathbf{x}}
\def\J{\mathbf{J}}
\def\D{\mathbf{D}}
\def\E{\mathbf{E}}
\def\S{\mathbf{S}}

\def\zerosup{\raisebox{-4pt}{\LARGE 0}}
\def\zeroinf{\raisebox{2pt}{\LARGE 0}}

\newcommand{\Frac}[2]{\displaystyle{\frac{#1}{#2}}}
%\newcommand{\Int}[2]{\displaystyle{\int\limits_{#1}^{#2}}}     
\newcommand{\Sum}[2]{\displaystyle{\sum\limits_{#1}^{#2}}}
\renewcommand{\part}{\partial \,}

% Comando per le dimensioni verticali degli array
\renewcommand{\arraystretch}{1.4}
% Variabili veloci da scrivere
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}
% Comando per i riferimenti
\newcommand{\refsec}[1]{\text{Sect.}\ref{#1}}
\newcommand{\reffig}[1]{\text{Fig.}\ref{#1}}
\newcommand{\reftab}[1]{\text{Tab.}\ref{#1}}


% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{proof}{Proof}[section]
\newtheorem{remark}{Remark}[section]

\newcommand{\unit}[1]{\mathrm{#1}}
\newcommand{\electronvolt}{\unit{eV}}
\newcommand{\kelvin}{\unit{K}}
\newcommand{\nano}{\unit{n}}
\newcommand{\meter}{\unit{m}}
\newcommand{\second}{\unit{s}}
\newcommand{\volt}{\unit{V}}
\newcommand{\grammi}{\unit{g}}
\newcommand{\Kg}{\unit{Kg}}
\newcommand{\coul}{\unit{Coul}}
\newcommand{\mol}{\unit{mol}}
\newcommand{\lit}{\unit{L}}
\newcommand{\Mol}{\unit{M}}
\newcommand{\C}{\unit{C}}
\newcommand{\farad}{\unit{F}}
\newcommand{\A}{\unit{A}}
\newcommand{\ohm}{\unit{\Omega}}

	
